Natural Is The Best: Model-Agnostic Code Simplification for Pre-trained Large Language Models

Pre-trained Large Language Models (LLM) have achieved remarkable successes in several domains. However, code-oriented LLMs are heavy in computational complexity, and quadratically with the length of the input. Toward simplifying the input program of an LLM, the state-of-the-art approach has the strategies to filter the input code tokens based on the attention scores given by the LLM. The decision to simplify the input should not rely on the attention patterns of an LLM, as these patterns are influenced by both the model architecture and the pre-training dataset. Since the model and dataset are part of the solution domain, not the problem domain where the input belongs, the outcome may differ when the model is pre-trained on a different dataset. We propose SlimCode, a model-agnostic code simplification solution for LLMs that depends on the nature of input code tokens. As an empirical study on the LLMs including CodeBERT, CodeT5, and GPT-4 for two main tasks: code search and summarization, we reported that 1) the removal ratio of code has a linear-like relation with the saving ratio on training time, 2) the impact of categorized tokens on code simplification can vary significantly, 3) the impact of categorized tokens on code simplification is task-specific but model-agnostic, and 4) the above findings hold for the paradigm-prompt engineering and interactive in-context learning. The empirical results showed that SlimCode can improve the state-of-the-art technique by 9.46% and 5.15% in terms of MRR and BLEU score on code search and summarization. Moreover, SlimCode is 133 times faster than the state-of-the-art approach. Additionally, SlimCode can reduce the cost of invoking GPT-4 by up to 24% per API query, while still producing comparable results to those with the original code.

==> irrelevant/firstParadigm.tex <==
\subsubsection{Experiments in fine-tune paradigm}
\label{sec:code-search-results}


\begin{table}[h]
\centering
\caption{Comparison of average remove percent, $MRR$ using codeBert and MRR using codeT5 for different code search scenarios.}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Code search} & \textbf{Ratio} & \textbf{CodeBert} & \textbf{CodeT5} \\
\hline
base methods & 0 & 0.743 & 0.749 \\
identifiers & 15.01\% & 0.650  & 0.683  \\
structure tokens & 11.76\% & 0.715  & 0.730  \\
simple symbols & 49.15\% & 0.722  & 0.729 \\
function invocation & 38.61\% & 0.682 & 0.698\\
function signature & 20.13\% & 0.649  & 0.680 \\
tokens in PDG & 33.75\% & 0.675 & 0.680 \\
\hline
\end{tabular}
\label{tab:code_search}
\end{table}

Here are some observations:
\begin{enumerate}
    \item As the removal ratio increases, the performance of both codeBert and codeT5 appropriately decreases. However, codeT5 outperforms codeBert at any removal ratio and has slower deterioration of performance.
    \item In code search tasks, identifier/simple symbols tokens have a greater/less impact than random tokens for both models. Furthermore, codeT5 outperforms codeBert as well.
    \item CodeBert/CodeT5 has a less/greater impact than random tokens. Moreover, codeT5 outperforms codeBert. (-2.94\% $>$ -4.31\%)
\end{enumerate}

Given a code description and a code method, code search task is to check if they are matched. In this scenario, the stronger the correlation between tokens in code descriptions and code methods, the higher the probability of similarity between the description and method. Thus, codeBert and codeT5 should put classification attentions on tokens with strong bimodal correlations, which form ‘cls’ for classification. Fortunately, tokens with strong bimodal correlations for classification are roughly learned in pre-training since MLM/BDG learn bimodal correlations for token prediction. The two bimodal correlations are similar.  (Transfer learning)

From the above experiment results, the attention rank of the classes of tokens for code search is shown as follows:
$$
Identifier > structure tokens > simple symbol
$$

More specifically, 
\begin{enumerate}
\item For Observation 1: 1) Many tokens with strong bimodal correlations remains even if removing some randonm tokens;2) codeT5 pre-trains more tokens with stronger correlations (bimodal dual generation $>$ MLM and MSP $>$RTD).

\item For Observation 2: 1) Usually identifiers/simple symbols usually are tokens with stronger/weaker bimodal correlations.2) codeT5 pre-trains more tokens with strong correlations. (more pre-training tasks)

\item For Observation 3:1)The structure tokens in codeT5 could be tokens with stronger bimodal correlations than the tokens in CodeBert because of MSP(Masked Span Prediction) and BDG (bimodal dual generation). CodeBert do not have such pre-training task for structure tokens. Thus, codeBert/ codeT5 has a less/greater impact than random tokens.
\end{enumerate}


\begin{table}[h]
\centering
\caption{Table Caption Goes Here}
\begin{tabular}{l|c|c|c}
\hline
\textbf{Code summarization} & \textbf{Ratio} & \textbf{codeBert} & \textbf{codeT5} \\
\hline
Base methods & 0 & 18.58 & 20.48 \\
identifiers & 16.34\% & 17.87 & 19.49 \\
structure tokens & 12.87\% & 18.47 & 20.34 \\
simple symbols* & 52.65\% & 18.57 & 20.38 \\
function invocation & 38.78\% & 18.17 & 20.31  \\
function signature & 18.05\% & 15.86& 16.61  \\
tokens in PDG & 30.61\% & 17.82 & 19.60 \\
\hline
\end{tabular}
\label{tab:code_summarization}
\end{table}

Here are some observations:
\begin{enumerate}
    \item As the removal ratio increases, the performance of both codeBert and codeT5 appropriately decreases. And codeT5 outperforms codeBert.
    \item Both models show that the use of random tokens has a greater effect than using identifiers. Furthermore, structure tokens and simple symbols have significantly less impact than random tokens. 
    \item Function signature tokens play an essential role in code summarization task. Taking them out would be equivalent to removing over half of the code.
\end{enumerate}
Again, code summarization has totally different from Code search. This process generates, rather than classifies. After considering all generated tokens, the decoder (encoder-decoder attention) should put attentions on most indicative tokens from the encoder to form the embedding of the next token. For codeT5,  how to ‘pick up’ indicative tokens is learned in the pre-train for the decoder by BDG.

Based on the experiment results, we have ranked the classes of tokens according to their relevance for code summarization.
$$
function signature >> identifiers >> structure tokens > function-signature tokens
$$

More specifically, 
\begin{enumerate}
\item For Observation 1: 1) Many indicative tokens remains even if even removing some random tokens. 2) codeT5 pre-trains more indicative tokens, the decoder of codeBert is not pre-trained model.

\item For Observation 2: Code descriptions usually provide an overview and rarely delve into details. Therefore, the function signature can be considered the "title" of the code description and has better inductive performance. Identifiers and structure tokens, on the other hand, refer to more details and lead to worse performance.

\item For Observation 3:xxxxxxxxxx
\end{enumerate}

\begin{figure}[t]
  \centering
  \includegraphics[width=8cm]{figures/codeBert-code2nl-BLEU4.pdf}
  \caption{The results of random token removal on code summarization dataset with CodeBert model.}
  \label{fig:overview}
\end{figure}
\begin{figure}[t]
  \centering
  \includegraphics[width=8cm]{figures/code2nl.pdf}
  \caption{The results of random token removal on code search dataset with CodeT5 model.}
  \label{fig:overview}
\end{figure}

==> irrelevant/secondParadigm.tex <==
\subsubsection{The results of experiments for code summarization}



==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motivation}
Pre-trained large language models can significantly aid users in code-related tasks. However, the usage of computing resources by these large models is also notorious. 
Generally, the amount of computing resources required is seriously depends on the number of tokens of the input to models, whether for fine-tuning or prediction. 
For instance, the pricing of GPT-4 for the number of tokens in the input is given here~\cite{openai-pricing}.

Code simplification is a practical way to reduce training and prediction time, while maintaining performance as much as possible. Given various pre-trained models and downstream tasks, it is intuitive that not all input tokens play critical roles in downstream-task fine-tuning or prediction. This is confirmed by experiments in the later section. 
For instance, when it comes to code search and summarization tasks, even eliminating around 50\% of tokens only results in a less than 3\% reduction in the performance of CodeBERT and CodeT5 models. 
Here an example of bubble sort demonstrates such cases with the two downstream tasks: code research and summarization.
The followings are the code of bubble sort and its description.
\newline
\newline
{\em The code of bubble sort:}
\begin{lstlisting}
def bubble_sort(arr):
    n = len(arr)
    for i in range(n - 1):
        for j in range(n - 1 - i):
            if arr[j] > arr[j + 1]:
                arr[j], arr[j + 1] = arr[j + 1], arr[j]
\end{lstlisting}
{\em The description of bubble sort:}
%\begin{quote}
    {\em "The method is a basic implementation of the bubble sort algorithm in Python. Bubble sort works by repeatedly swapping adjacent elements if they are in the wrong order until the entire array is sorted."}
%\end{quote}

For code search, the model checks whether the code and the description match by utilizing the embeddings of tokens in both documents.
During pre-training or fine-turning, the model learns the correspondence between two or more tokens. 
As a result, if the vectors of two tokens are close, the tokens are more likely to be correspondent. 
For instance, \code{bubble\_sort} in the code corresponds both "bubble" and "sort" in the description, 
and the code \code{arr} correspond "array" in the description as well.
In contrast, tokens like \code{+}, \code{=}, and \code{if} have no clear corresponding tokens in the description. Therefore, removing them in this example does not significantly affect the matching results since they cannot provide direct "hints".

For code summarization, a description of the given code is automatically generated. Similarly, not all tokens in the code are equally important for generating the summary. Function names and variables play crucial roles since they could have correspondences in the generated text and provide more guidance or "hints" for token generation. In contrast, tokens such as \code{+} and \code{=} are considered trivial since they have no obvious respective tokens in the description. 

In short, for downstream tasks, the more “hints" a token provides, the more it needs to be preserved here.
In fact, tokens with hints can be used across models or are even downstream tasks. For instance, both CodeBERT and CodeT5 learn the correspondence for potential tokens in bimodal data (such as \code{bubble\_sort} and "sort") during pre-training. Meanwhile, function names like \code{bubble\_sort} provide strong hints for solving both tasks.

To identify and preserve tokens carrying more hints, one effective strategy is to categorize them based on their inherent properties, e.g., 
 lexical, grammatical, and semantic attributes. 
Tokens with "hints" are typically important at the lexical, syntactic, semantic, or all levels.
Thus, we classify tokens according to their importance at different levels, with higher- and lower-importance tokens being retained or removed, respectively. This is the reason for \underline{RQ(2-4)} .
For instance, at the lexical level, variables are much more important than operators; thus, operators should be removed before variables.

Based on what we learned from \underline{RQ(2-4)}, we should offer a lightweight method for simplifying code using categorized tokens (\underline{RQ-5}). This method allows users to quickly remove tokens and reduces the need for computing the source, unlike the model-dependent code simplification method~\cite{dietcode-fse22}.

